A single-spin precessing gravitational wave in closed form

In coming years, gravitational wave detectors should find black hole-neutron star binaries, potentially coincident with astronomical phenomena like short GRBs. These binaries are expected to precess. Gravitational wave science requires a tractable model for precessing binaries, to disentangle precession physics from other phenomena like modified strong field gravity, tidal deformability, or Hubble flow; and to measure compact object masses, spins, and alignments. Moreover, current searches for gravitational waves from compact binaries use templates where the binary does not precess and are ill-suited for detection of generic precessing sources. In this paper we provide a closed-form representation of the single-spin precessing waveform in the frequency domain by reorganizing the signal as a sum over harmonics, each of which resembles a nonprecessing waveform. This form enables simple analytic calculations (e.g., a Fisher matrix) with easily-interpreted results. We have verified that for generic BH-NS binaries, our model agress with the time-domain waveform to 2\%. Straightforward extensions of the derivations outlined here [and provided in full online] allow higher accuracy and error estimates.

==> python/spintaylor_f2_t2_faithfulness <==
#! /usr/bin/env python

import lal as lal
import lalsimulation as lalsim
import numpy as np
from numpy.fft import fft, ifft
from numpy import array, arange, sqrt, log, pi, cos, sin, arccos, dot
from random import uniform
import sys

# Author: Andrew Lundgren
# Email: andrew.lundgren@ligo.org

# DOCUMENTATION
# This code demonstrates numerically that the SpinTaylorF2 waveform is sufficiently faithful to SpinTaylorT2. It can be used as a module 
# If using this function as a module:
# td_fd_faithfulness(mass1, mass2, inclination, chi1x, chi1y, chi1z, phi0)
# mass1: mass of the spinning object (usually BH) in units of Msol
# mass2: mass of the second object (usually NS) in units of Msol
# inclination: initial inclination 

# INSTALLATION OF SUPPORT CODE
#   lalsuite instructions:
#           + install LIGO support software.  For mac,
   #      https://www.lsc-group.phys.uwm.edu/daswg/docs/howto/macports.html
   #      Run
   #      	port install lscsoft-deps
   #      	port install glue
   #      	port install swig-python
   # + install lalsuite
   #      git clone git:/ligo-vcs.phys.uwm.edu/lalsuite.git
   #      cd lalsuite
   #      mkdir build_all
   #      ./00boot
   #      cd build_all
   #      ../configure --prefix=${HOME}/LIGO/Packages/analysis --enable-swig-python --enable-mpi
   #      make && make install
# 5: Configure your environment variables
# Add the following to your .bash_profile
# LAL_LOCATION=${HOME}/LIGO/Packages/analysis
# source ${LAL_LOCATION}/etc/lal-user-env.sh          # can be different
# source ${LAL_LOCATION}/etc/lalframe-user-env.sh
# source ${LAL_LOCATION}/etc/lalinspiral-user-env.sh
# source ${LAL_LOCATION}/etc/lalsimulation-user-env.sh



# Numerical constants
mtsun = lal.LAL_MTSUN_SI
dyn_range_fac = 2.0**69.0
distance = 1.e6*lal.LAL_PC_SI # Put the source at a Mpc

# PN order of non-spinning and spinning terms in the phasing
pn_order = 7
spin_order = 5
pn_flags = lalsim.SimInspiralCreateWaveformFlags()
lalsim.SimInspiralSetSpinOrder(pn_flags, spin_order)

# Names of the approximants we are using
fd_approx = lalsim.SpinTaylorF2
td_approx = lalsim.SpinTaylorT2

# Choices for frequencies and sample rates
f_inj = 14.0 # Start the injection
f_min = 15.0 # Start the overlap calculation
sample_rate = 4096 
len_sig_secs = 512
N = len_sig_secs * sample_rate
dt = 1.0 / sample_rate
df = 1.0 / len_sig_secs

# PSD and inverse PSD 
def psd(ff):
	return dyn_range_fac*dyn_range_fac*lalsim.SimNoisePSDaLIGOZeroDetHighPower(ff)

f_min_idx = int(f_min / df)
invpsd = np.concatenate((np.zeros(f_min_idx), [1.0/psd(f) for f in df * arange(f_min_idx,N)]))

# Vector tools
def norm(vec):
	return sqrt(dot(array(vec),array(vec)))

def random_vec(min_mag, max_mag):
	""" Randomly oriented vector with magnitude in [min_mag, max_mag] """
	costheta = uniform(-1.,1.)
	sintheta = sqrt(1.-costheta*costheta)
	phi = uniform(0.,2.*pi)
	vec = array([costheta, sintheta*cos(phi), sintheta*sin(phi)])
	vec *= uniform(min_mag, max_mag)
	return vec

def chi_kappa(m1, m2, inclination, chi1):
	"""Transform from SpinTaylor frame to chi, kappa"""
	mtot = m1+m2
	eta  = m1*m2/(mtot*mtot)
	chi1 = array(chi1)
	angfac = lambda f: (m1*m2) / pow(pi*mtsun*mtot*f,1.0/3.0)
	Lhat = array([sin(inclination), 0.0, cos(inclination)])
	Jtot = angfac(f_inj) * Lhat + m1*m1*chi1
	kappa = dot(Lhat,chi1) / max(norm(chi1),1.0e-6)
	return (norm(chi1), kappa)

# Padding TD and FD to prevent numerical problems
def inject(inj_arr):
	""" Inject a TD waveform into the middle of the segment """
	signal = np.zeros(N)
	start_idx = N/2 - len(inj_arr)
	for idx, val in enumerate(inj_arr, start_idx):
		signal[idx] = dyn_range_fac * val
	return fft(signal)

def pad_fseries(fseries, length):
	""" Pad FD waveform with zeros up to the Nyquist frequency """
	return np.concatenate( (fseries, np.zeros(N-len(fseries))) )

# Functions to make the TD and FD signals
def make_td_signal(mass1, mass2, inclination, chi1x, chi1y, chi1z, psi, phi0, approximant=td_approx):
	""" Make TD waveform using standard SpinTaylor coordinates """
	hpc, hxc = lalsim.SimInspiralChooseTDWaveform( \
					phi0, dt, \
					mass1 * lal.LAL_MSUN_SI, mass2 * lal.LAL_MSUN_SI, \
					chi1x, chi1y, chi1z, \
					0.0, 0.0, 0.0, \
					f_inj, 0., distance, inclination, \
					0.0, 0.0, pn_flags, None, \
					0, pn_order, approximant)

	waveform = array(hpc.data.data)*cos(2.*psi) + array(hxc.data.data)*sin(2.*psi)

	return inject(waveform)

def make_fd_signal(mass1, mass2, inclination, chi1x, chi1y, chi1z, psi, phi0, approximant = fd_approx):
	""" Make FD waveform using standard SpinTaylor coordinates. Should be faithful to TD waveform """
	hptilde, hxtilde = lalsim.SimInspiralChooseFDWaveform( \
							phi0, df, \
							mass1 * lal.LAL_MSUN_SI, mass2 * lal.LAL_MSUN_SI, \
							chi1x, chi1y, chi1z, \
							0.0, 0.0, 0.0, \
							f_inj, 0., distance, inclination, \
							0.0, 0.0,  pn_flags, None, \
							0, pn_order, approximant)

	htilde = array(hptilde.data.data)*cos(2.*psi) + array(hxtilde.data.data)*sin(2.*psi)

	return pad_fseries(htilde, N)

# Functions for overlap computation
def f_isco(mtot):
	""" Usual Schwarzschild ISCO cutoff v = 1/sqrt(6) """
	return 4400. / mtot

def sigma(htilde, f_max):
	""" Waveform normalization """
	f_max_idx = int(f_max / df)
	integrand = htilde * htilde.conjugate() * invpsd
	sigmasq = np.sum(np.abs(integrand[f_min_idx:f_max_idx]))

	return sqrt(sigmasq)

def overlap(stilde, htilde, f_max):
	""" Overlap, maximized over time and phase

	Return overlap, phase mismatch in degrees, time offset in seconds """
	f_max_idx = int(f_max / df)
	integrand = stilde * htilde.conjugate() * invpsd
	for idx in range(f_max_idx,len(integrand)):
		integrand[idx] = 0.0
	temp = ifft(integrand)
	maxidx = np.argmax(np.abs(temp))
	return (N * abs(temp[maxidx]) / (sigma(stilde, f_max)*sigma(htilde, f_max)), 180./pi*np.angle(temp[maxidx]), maxidx*dt - len_sig_secs/2.)

# This is the central function that calculates the faithfulness
def td_fd_faithfulness(mass1, mass2, inclination, chi1x, chi1y, chi1z, psi, phi0):
	""" Calculate faithfulness of SpinTaylorT2 versus SpinTaylorF2

	Returns tuple of (plus, cross) waveform faithfulness. Uses standard SpinTaylor coordinates. """
	stilde1 = make_td_signal(mass1, mass2, inclination, chi1x, chi1y, chi1z, psi, phi0)
	stilde2 = make_fd_signal(mass1, mass2, inclination, chi1x, chi1y, chi1z, psi, phi0)
	olap, _, _ = overlap(stilde1, stilde2, f_isco(mass1+mass2))

	return olap

# Command line interface
if __name__ == "__main__":

	if len(sys.argv) < 3:
		print "Computes the faithfulness of the SpinTaylorF2 model against the SpinTaylorT2 model. See comments in the file for more information." 
		print "Args: output_filename.dat num_overlaps"
		sys.exit()
	else:
		fname = sys.argv[1]
		num_overlaps = int(sys.argv[2])

	fout = open(fname, 'w')
	fout.write("# mass1 mass2 inclination chi1x chi1y chi1z psi phi0 chi kappa faithfulness\n")

	num_queued = 0
	queue = []
	for idx in xrange(num_overlaps):
		# Change these lines to simulate another distribution
		mass1 = 10.
		mass2 = 1.4
		inclination = arccos(uniform(-1.,1.))
		psi = uniform(0.,2.*pi)
		phi0 = uniform(0.,2.*pi)
		chi1x, chi1y, chi1z = random_vec(0.5, 1.0)
		chi, kappa = chi_kappa(mass1, mass2, inclination, [chi1x,chi1y,chi1z])

		olap = td_fd_faithfulness(mass1, mass2, inclination, chi1x, chi1y, chi1z, psi, phi0)

		queue.append("%.4f %.4f %.6f %.6f %.6f %.6f %.6f %.6f %.4f %.4f %.4f\n" % (mass1, mass2, inclination, chi1x, chi1y, chi1z, psi, phi0, chi, kappa, olap))
		num_queued += 1
		if num_queued >= 50:
			fout.write("".join(queue))
			fout.flush()
			queue = []
			num_queued = 0

	fout.write("".join(queue))
	fout.close()


